A Phenomenological AI Foundation Model for Physical Signals

The objective of this work is to develop an AI foundation model for physical signals that can generalize across diverse phenomena, domains, applications, and sensing apparatuses. We propose a phenomenological approach and framework for creating and validating such AI foundation models. Based on this framework, we developed and trained a model on 0.59 billion samples of cross-modal sensor measurements, ranging from electrical current to fluid flow to optical sensors. Notably, no prior knowledge of physical laws or inductive biases were introduced into the model. Through several real-world experiments, we demonstrate that a single foundation model could effectively encode and predict physical behaviors, such as mechanical motion and thermodynamics, including phenomena not seen in training. The model also scales across physical processes of varying complexity, from tracking the trajectory of a simple spring-mass system to forecasting large electrical grid dynamics. This work highlights the potential of building a unified AI foundation model for diverse physical world processes.

==> formulation.tex <==
Imagine an electrical motor whose behavior can be described in terms of temperature, electrical current, rotation speed, vibration, torque etc. We denote each such physical quantity as $q_i(t)$ and a set of all the physical quantities that describe a particular object or process as $Q = \cup_i q_i(t)$. It's reasonable to think that the physical world can be represented as a collection of physical quantities $Q$ that vary over space and time. We call that superset of all physical quantities as $\Omega = \cup Q$.

We ask whether there is a single phenomenological model for all $q_i \in \Omega$, i.e. a compact representative model that is capable of both describing the past trajectory and predicting future trajectory of $q(t)$, similar to how the differential equation for a pendulum can be used for both representing its past trajectory as well as predicting its future motion. In other words, we seek a compressed representation of $q_i(t)$ that both describes $q(t_i')$ for $t' \leq t$ and predicts $q_i(t')$ for $t' > t$, for all $t$ and $q_i \in \Omega$.

%\begin{figure}
%    \centering
%    \includegraphics[width=0.9\linewidth]{figures/phenomenological_model.png}
%   \caption{[Placeholder figure] A phenomenological model describes past measurements ($t<t'$) and predicts future measurements ($t>t'$) for all possible values of $t'$.}
%    \label{fig:phenomenological_model}
%\end{figure}

The challenge is that neither the physical quantities $q(t)$ nor their governing laws are inherently known, nor can the true underlying distribution of these physical quantities, denoted $p_{q_i}(q_i)$ be directly sampled. The physical quantities can only be indirectly observed through sensors which measure a subset of physical quantities and which introduce noise and bias due to the operational characteristics of the sensor (i.e. transfer function). Thus the measurements are incomplete, stochastic observations of the true underlying continuum of physical quantities. This is a well-known philosophical standpoint, espoused most famously by Michael Scriven and Nancy Cartwright: that any so-called “physical law” is at best an approximation of the truth [REF].

Let’s denote the observation of quantity $q_i(t)$ using sensor $s_j$ as $m_{i,j}(t)$. The sensor can be fully characterized by the conditional probability $p_{m_{i,j}|q_i}(m_{i,j}|q_i)$, which describes the distribution of the measurement values given the true (unknown) quantity. This conditional pdf therefore abstracts all the characteristics inherent to any sensor, i.e. transfer function, noise, linearity, etc, see [REF, REF] for details.  The true underlying distribution of $q_i$ is described by $p_{q_i}(q_i)$, which is unknown and cannot be directly sampled.

The probability distribution function of $m_{i,j}(t)$ is then given by $p_{m_{i,j}}(m_{i,j}) = \int_q p_{m_{i,j}|q_i}(m_{i,j}|q_i) p_{q_i}(q_i) dq$. 

We formulate the phenomenological model as a mapping $f: m_{i,j}(t) \rightarrow w_{i,j}$ that enables mappings $g_-: w_{i,j} \rightarrow m_{i,j}'(t'), t'\leq t$ and $g_+: w_{i,j} \rightarrow m_{i,j}'(t'), t' > t$
for all $q_i \in \Omega$ and sensor $p_{m_{i,j}|q_i}(m_{i,j}|q_i)$.


==> introduction.tex <==
This work is motivated by the challenges of applying Artificial Intelligence (AI) to interpret real-time physical signals, a critical requirement for addressing complex, real-world problems that require the design and training of ``physically correct'' AI models. Examples include monitoring and managing large-scale infrastructure systems such as transportation networks, improving energy efficiency in electrical grids to address climate-related challenges \cite{Akomea-Frimpong2023}, enabling data-driven experimental scientific discoveries \cite{Wang2023}, advancing novel human-computer interaction techniques%like spatial interaction
, and others.

A common approach to designing ``physically correct'' AI models involves incorporating strong inductive biases or ``first principles'', such as the conservation of energy \cite{Liu2021, Greydanus2019}. Extensive research has explored inductive bias techniques for tasks such as physical scene understanding, recovering latent physical properties, learning physics simulators, discovering physical concepts, and designing physics engines and adaptive inference agents, among many others.

While powerful, the first-principles approach leads to highly specialized AI models that are difficult to generalize or scale to other use cases. For instance, an AI model designed to analyze fluid motion would incorporate the Navier-Stokes equations \cite{Raissi2020} and could not be applied to interpreting radar Doppler images in human-computer interaction scenarios \cite{Hayashi2021}. More importantly, physically accurate mathematical models are impractical in many real-world systems due to their complexity and the influence of external factors that cannot be easily captured by a closed set of equations. For example, the behavior of large electrical grids is influenced not only by the specifics of electrical system design but also by external factors such as weather conditions.

\textit{Representative} or \textit{phenomenological} models \cite{Bas2008} address the limitations of first-principles approaches by training AI models on large datasets of physical system measurements, allowing for the inference of physically correct interpretations without incorporating prior knowledge of physical laws \cite{Iten2020}. These models have proven highly successful in solving complex real-world problems across various domains and handling different types of sensor data, from simple one-dimensional signals, such as using accelerometer data to analyze human gait, to discovering pulsars from complex multidimensional radio telescope measurements \cite{Zhu2014}.

However, scalability remains a significant challenge for phenomenological AI models, similar to the strong inductive models discussed earlier. The applicability of representative models is fundamentally constrained by the availability of training data, which can be difficult, expensive, or even impossible to acquire due to security, privacy, and proprietary concerns, among others. Additionally, these models are highly sensitive to variability in sensor characteristics and the specifics of the signal processing chain used for data preprocessing. Even minor variations in sensor properties often necessitate recollecting data and retraining the models. As a result, these models tend to be highly specialized, narrowly designed to solve specifi-c problems, and are typically not generalizable across different sensors or system configurations.

The current highly fragmented approach to building and deploying AI solutions in the physical world remains labor-intensive, technically demanding, and resource-intensive, creating  substantial barriers and costs for implementing AI in numerous impactful and critical real-world applications. As a result, many practical problems remain unsolved, and numerous opportunities are underdeveloped due to the associated costs and technical complexities involved in AI deployment.

In this paper, we propose a novel framework for developing AI models that can be \textit{universally applied to physical processes of any nature}, which we refer to as the $\Omega$ framework. Our framework is based on a phenomenological methodology, meaning that no prior physical knowledge or inductive bias is introduced. The aim is to construct a single, versatile foundational physical AI model capable of generalizing across diverse physical domains,  applications, and physical sensing apparatuses. This work is inspired by recent advancements in natural language processing, where generative models based on transformer architectures, such as GPT-4, have demonstrated that a single model trained on a vast corpus of text can encode the general structure of languages and, consequently, perform as well as or better than narrow specialized models across a wide range of tasks. Proposing the $\Omega$ framework is the primary contribution of this paper.

While foundational models have demonstrated significant potential in domains such as language processing, image analysis, and general time series data, to the best of our knowledge, there has been limited research investigating whether these models can be effectively applied to physical sensor-based data. Specifically, it remains unclear whether such models can achieve performance comparable to existing approaches for one-dimensional, time-varying sensor signals, which are typical in measuring complex physical processes. In this work, we present the design of a foundational model implementing the $\Omega$-framework, trained on 3.5 million examples of physical measurements covering a diverse range of real-world processes. The design and demonstration of this model constitute the second contribution of this paper.

A systematic experimental validation demonstrated the model's ability to accurately describe kinematic, thermodynamic, and electromagnetic processes from real, canonical physical systems not included in the training data. To further assess our framework, we applied it to complex real-world physical processes, such as household electrical consumption, the solar spot index, and daily temperature variations in Delhi. Despite none of these processes being represented in the training dataset, the $\Omega$-trained phenomenological model was able to accurately forecast the behavior of these systems, with an error rate within 12\% of a model specifically trained on the target system.

Although previous efforts have explored the application of transformer-based models for multimodal data, including general time-series data \cite{Das2024, Girdhar2023}, they have not systematically validated whether these models can produce physically valid behaviors, either in classic physical experiments or complex real-world systems. A thrid contribution of this paper is the validation of our framework, demonstrating its generalization capabilities across a wide range of physical processes.

The remainder of this paper details the $\Omega$-framework, the design of the foundation model, and the results of our experimental evaluations.

==> model.tex <==
This section presents the design and training of the model that we implemented to explore possibility of universal model for physical world based on the $\Omega$ framework. We provide a high-level overview of the architecture, more details can be found in the Appendix.

The model architecture is illustrated in Figure \ref{fig:model_high_level}. Sensor measurements are encoded as temporal sequences of one-dimensional patches of fixed length, which are projected into a unified embedding space by utilizing a standard transformer architecture \cite{vaswani2017attention, dosovitskiy2021}. The transformer architecture preserves the deep temporal structure of individual patches, and as the encoder is trained on large, diverse sets of sensor data, it effectively learns the underlying temporal patterns of a wide range of complex physical processes, regardless of the specific sensor modality. 

The resulting compact, universal representation can then be employed with relatively small task-specific decoders, including \textit{trajectory following} or \textit{forecasting} and \textit{reconstruction} (Figure \ref{fig:model_high_level}). These decoders corresponds to the $g_-$ and $g_+$ mapping functions we defined in Equation \ref{eq:mappins}.

       \begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/model_high_level.pdf}
    \caption{Model Architecture: The sensor data is normalized and segmented into a set of fixed-length, one-dimensional patches that are are used to train a transformer-based encoder network in a self-supervised manner. Compact downstream decoders are then employed to reconstruct and predict the trajectories of the physical quantities of interest.}
    \label{fig:model_high_level}
\end{figure}


\subsection{Encoder for physical quantities}

Encoder projects sensor data into universal latent representation by training the transformer-based network on wide variety of diverse physical data. 

\paragraph{Patching.} Each physical quantity $q_i$ measured using sensor $s_j$ is represented as a set of $m$ time-varying measurements $\{s_1(t),...,s_m(t)\}$ and scale each measurement context to the range [0,1]. Each measurement $s_i$ is then segmented into a sequence of $n$ patches $S_i = \bigcup_{j=1}^{n} \{ p_{i,j} \}$, with $p_{i,j} \in \mathbb{R}^{l_{patch}}$. Following related work where fixed patch sizes were used for images \cite{dosovitskiy2020image} and, unlike traditional signal processing approaches [ref], we do not adjust the resolution of the patches to match the sampling frequency of the measurements, which expands the amount of available data and simplifies ingestion by the model. 

\paragraph{Projection to the embedding space} The sensor patches are projected into the embedding space of dimension $d_{model}$ using a linear layer, resulting in a sequence of $n$ patch embeddings $T_i = \bigcup_{j=1}^n \{t_{i,j}\}$. A positional embedding $q_j \in \mathbb{R}^{d_{model}}$ is added to each patch embedding $t_{i,j}$ to capture the temporal order of the patches and is learned during training [REF]. Finally, we append one learnable \texttt{[SEQ]} token \footnote{Wich represents the full input sequence in a single embedding, analogous to the\texttt{[CLS]} token in \cite{devlin2018bert,dosovitskiy2020image}.} to the patch embeddings, resulting in the final sequence $ Z_i = \bigcup_{j=1}^{n+1} \{ z_{i,j} \}$. %, which is the input to the transformer.

\paragraph{Encoder architecture} 

  We use a vanilla transformer \cite{vaswani2017attention} with 6 layers of alternating causal multi-head attention heads and feedforward layers. The output of the attention is projected by a learnable linear layer, batch normalized and summed with residual connections; and  the feedforward network is an MLP. \footnote{See Appendix \ref{sec:appendix}for a detailed description of the architecture.} The output of the transformer is a sequence of embeddings $Z_i^{\text{emb}} = \bigcup_{j=1}^{n+1} \{z_{i,j}^{\text{emb}}\}$ from which we extract the $(n+1)$th one, corresponding to the location of the appended \texttt{[SEQ]} token. This embedding vector constitutes a representation of the full input sequence. %The analogy from other modalities is that the output embedding for the [CLS] token is used for sentence-level meaning classification in BERT and image-level classification in ViT. 



\subsection{Task-specific decoders }


The embedding vector $Z^{\text{emb}}_{i, n+1}$ is then input into task-specific decoders. In this work, we examine two exemplar tasks: reconstruction and forecasting. Both decoders are lightweight MLPs with the same architecture, except for the dimensionality of the intermediate and last layers. A similar architecture can be used for other tasks such as classification. The motivating idea is that the encoder should capture and represent the salient information in the sensor measurement, allowing the downstream task-specific decoders to have a relatively small number of parameters and making them easily trainable. For a detailed description of the decoders' architecture, see Appendix \ref{sec:appendix}. 
%The decoder MLP architecture consists of a layer normalization step, a learnable linear layer $\mathbf{W}_{d,1} \in \mathbb{R}^{d_\text{model} \times d_\text{int}}$, ReLU activation, and a second learnable linear layer $\mathbf{W}_{d,2} \in \mathbb{R}^{d_\text{int} \times d_\text{out}}$. The intermediate dimension $d_\text{int}$ and output dimension $d_\text{out}$ vary according to the task. For reconstruction, $d_\text{out}$ is equal to the number of points in the input measurement, $d_\text{out} = nl_\text{patch}$ and $d_\text{int} = \frac{d_\text{out}}{2}$. For forecasting, $d_\text{int} = d_\text{model}$ and $d_\text{out} = l_\text{pred}$ where $l_\text{pred}$ denotes the desired length of the prediction window.

\subsection{Training and evaluation}

\paragraph{Training} We use a collection of publicly available datasets from a wide variety of physical domains and sensors. In particular, we leverage the LOTSA \cite{woo2024lotsa} datasets from physical domains (labeled as Energy, Climate, Nature, and Transport) and we discard datasets from non-physical domains \footnote{We recognize the unclear distinction between "physical" and "non-physical" data and plan to address this in future work, while encouraging the community to do the same.} (labeled as Healthcare, Econ/Finance, Web, Sales, and CloudOps) for our training set. In total, our training set comprises 290,753,280 observations (see appendix \ref{sec:appendix} for a detailed description). We use forecasting as the encoder pre-training task, enabling fully self-supervised training. The encoder and forecasting decoder are trained end-to-end using the mean square error (MSE) between the forecast and the true values of the sensor measurements as the loss function.
% We also performed early experiments using reconstruction of randomly masked patches within the sequence as the pre-training task, but obtained inferior results. We should revisit this again in future work, comparing both encoder pre-training approaches across a broader range of downstream tasks.
We use a batch size of 1024, learning rate of 1e-3, with an AdamW optimizer. On a single Nvidia A100 GPU, model pre-training takes 6 hours. To train the other task-specific decoders, we started from the frozen pre-trained encoder and train the decoder using the training set described above.
